ANNaMo: Coarse-grained modelling for folding and assembly of RNA and DNA systems

The folding of RNA and DNA strands plays crucial roles in biological systems and bionanotechnology. However, studying these processes with high-resolution numerical models is beyond current computational capabilities due to the timescales and system sizes involved. In this article, we present a new coarse-grained model for investigating the folding dynamics of nucleic acids. Our model represents 3 nucleotides with a patchy particle and is parametrized using well-established nearest-neighbor models. Thanks to the reduction of degrees of freedom and to a bond-swapping mechanism, our model allows for simulations at timescales and length scales that are currently inaccessible to more detailed models. To validate the performance of our model, we conducted extensive simulations of various systems: We examined the thermodynamics of DNA hairpins, capturing their stability and structural transitions, the folding of an MMTV pseudoknot, a complex RNA structure involved in viral replication, and also explored the folding of an RNA tile containing a k-type pseudoknot. Finally, we evaluated the performance of the new model in reproducing the melting temperatures of oligomers and the dependence on the toehold length of the displacement rate in toehold-mediated displacement processes, a key reaction used in molecular computing. All in all, the successful reproduction of experimental data and favorable comparisons with existing coarse-grained models validate the effectiveness of the new model.

==> tables/mismatch.tex <==

    \centering
    \begin{tabular}{cccc}
    \hline
        Mismatch & oxDNA & nNxB & $|\Delta|$ \\ \hline
        DNAh1:5-CGCAACCTCTTCGATGCG-3 & 53 & 56 & 3 \\ \hline
        DNAh2: 5-CGCAACCTCTTCGTTACG-3 & 40 & 19 & 21 \\ \hline
        DNAh3: 5-AACCGCCTCTTCGCGGCT-3 & 66 & 58 & 8 \\ \hline
        DNAh4: 5-AACCGCCTCTTCGAGGTT-3 & 25 & 39 & 14 \\ \hline
        DNAh5: 5-TCCGAGCTCTTCCTCGCA-3 & 53 & 36 & 17 \\ \hline
        DNAh6: 5-TCCGAGCTCTTCCTGGGA-3 & 39 & 34 & 5 \\ \hline
        DNAh7: 5-GAGTCCCTCTTCGGACAC-3 & 53 & 41 & 12 \\ \hline
        DNAh8: 5-GAGTCCCTCTTCGTACTC-3 & 37 & 32 & 5 \\ \hline
        DNAh9: 5-CCTGCACTCTTCTGTAGG-3 & 38 & 35 & 3 \\ \hline
        DNAh10: 5-CCTGCACTCTTCTGCAGC-3 & 60 & 48 & 12 \\ \hline
        DNAh11: 5-GCACCTCTCTTCAGGTGT-3 & 58 & 54 & 4 \\ \hline
        DNAh12: 5-GCACCTCTCTTCAGCTGC-3 & 42 & 27 & 15 \\ \hline
        ~ & ~ & ~ & ~ \\ \hline
        ~ & ~ & ~ & $\langle|\Delta|\rangle$ \\ \hline
        ~ & ~ & ~ & 9.9 \\ \hline
    \end{tabular}

